Transfer Entropy in MDPs with Temporal Logic Specifications

Emerging applications in autonomy require control techniques that take into account uncertain environments, communication and sensing constraints, while satisfying highlevel mission specifications. Motivated by this need, we consider a class of Markov decision processes (MDPs), along with a transfer entropy cost function. In this context, we study highlevel mission specifications as co-safe linear temporal logic (LTL) formulae. We provide a method to synthesize a policy that minimizes the weighted sum of the transfer entropy and the probability of failure to satisfy the specification. We derive a set of coupled non-linear equations that an optimal policy must satisfy. We then use a modified Arimoto-Blahut algorithm to solve the non-linear equations. Finally, we demonstrated the proposed method on a navigation and path planning scenario of a Mars rover.

==> App1.tex <==
We first prove the following lemma.
\begin{lemma}
\label{lemcoding}
For each $T=1, 2, ...$, we have
\[
I(\bar{X}^{T} \rightarrow W^{T} || U^{T-1},\tilde{X}^{T}) \geq I(\bar{X}^{T} \rightarrow U^{T} || \tilde{X}^{T}).
\]
\end{lemma}
\begin{proof}
The result is established by the following chain of inequalities.
\begin{align*}
&  I(\bar{X}^T \rightarrow W^T || U^{T-1},\tilde{X}^T) - I(\bar{X}^T \rightarrow U^T || \tilde{X}^T)  \\
& = \sum_{t=0}^T I\left(\bar{X}^t;W_t|W^{t-1},U^{t-1},\tilde{X}^t \right) - I\left(\bar{X}^t;U_t|U^{t-1},\tilde{X}^t \right)\\
& \stackrel{\text{(a)}}{=} \sum_{t=0}^T I\left(\bar{X}^t;W_t,U_t|W^{t-1},U^{t-1},\tilde{X}^t \right) \\
& \hspace{10ex}- I\left(\bar{X}^t;U_t|U^{t-1},\tilde{X}^t \right)\\
& \stackrel{\text{(b)}}{=} \sum_{t=0}^T I\left(\bar{X}^t;W^t|U^{t},\tilde{X}^t \right) - I\left(\bar{X}^t;W^{t-1}|U^{t-1},\tilde{X}^t \right)\\
& \stackrel{\text{(c)}}{=} \sum_{t=0}^T I\left(\bar{X}^t;W^t|U^{t},\tilde{X}^t \right) - I\left(\bar{X}^{t-1};W^{t-1}|U^{t-1},\tilde{X}^t \right)\\
& \stackrel{\text{(d)}}{\geq} \sum_{t=0}^T I\left(\bar{X}^t;W^t|U^{t},\tilde{X}^t \right) - I\left(\bar{X}^{t-1};W^{t-1}|U^{t-1},\tilde{X}^{t-1} \right)\\
& \stackrel{\text{(e)}}{=} I\left(\bar{X}^T;W^T | U^T,\tilde{X}^T \right) \geq 0. 
\end{align*}
Equality (a) holds since
\begin{align*}
&I(\bar{X}^t; W_t, U_t|W^{t-1}, U^{t-1}, \tilde{X}^t)=\\
&I(\bar{X}^t; W_t|W^{t-1}, U^{t-1}, \tilde{X}^t)
+I(\bar{X}^t; U_t|W^t, U^{t-1}, \tilde{X}^t)
\end{align*}
and the second term is zero since $U_t$ is conditionally independent of $\bar{X}^t$ given $(W^t, U^{t-1})$. Equality (b) can be shown by applying the chain rule for mutual information in two different ways:
\begin{align*}
&I(\bar{X}^t; W^t, U_t|U^{t-1}, \tilde{X}^t) \\
&=I(\bar{X}^t; W^{t-1}|U^{t-1}, \tilde{X}^t)+I(\bar{X}^t; W_t, U_t| W^{t-1}, U^{t-1}, \tilde{X}^t) \\
&=I(\bar{X}^t; U_t|U^{t-1}, \tilde{X}^t)+I(\bar{X}^t;W^t|U^t, \tilde{X}^t).
\end{align*}
Equality (c) holds since
\begin{align*}
&I(\bar{X}^t; W^{t-1}|U^{t-1}, \tilde{X}^t)=\\
&I(\bar{X}^{t-1}; W^{t-1}|U^{t-1}, \tilde{X}^t)+I(\bar{X}_t; W^{t-1}|U^{t-1}, \tilde{X}^t, \bar{X}^{t-1})
\end{align*}
and the second term is zero. To see (d), apply the chain rule in two different ways:
\begin{align*}
&I(\bar{X}^{t-1}, \tilde{X}_t; W^{t-1}|U^{t-1},\tilde{X}^{t-1}) \\
&=I(\tilde{X}_t; W^{t-1}|U^{t-1}, \tilde{X}^{t-1})+I(\bar{X}^{t-1}; W^{t-1}|U^{t-1}, \tilde{X}^t) \\
&=I(\bar{X}^{t-1}; W^{t-1}|U^{t-1}, \tilde{X}^{t-1}) \\
&\hspace{5ex}+I(\tilde{X}_t;W^{t-1}|U^{t-1},\tilde{X}^{t-1}, \bar{X}^{t-1}).
\end{align*}
Since the last term is zero, we have 
\[
I(\bar{X}^{t-1}; W^{t-1}|U^{t-1}, \tilde{X}^{t-1}) \geq I(\bar{X}^{t-1}; W^{t-1}|U^{t-1}, \tilde{X}^t).
\]
Finally, (e) is due to the telescopic cancellation.
\end{proof}

Theorem~\ref{theorate} can now be shown as
\begin{align*}
R&=\sum_{t=0}^{T-1} R_t \\
&\stackrel{\text{(a)}}{\geq} \sum\nolimits_{t=0}^{T-1} H(W_t) \\
&\stackrel{\text{(b)}}{\geq} \sum\nolimits_{t=0}^{T-1} H(W_t|W^{t-1}, U^{t-1}, \tilde{X}^t) \\
&\stackrel{\text{(c)}}{\geq} \sum\nolimits_{t=0}^{T-1} H(W_t|W^{t-1}, U^{t-1}, \tilde{X}^t) \\
&\hspace{10ex}-H(W_t|\bar{X}^t, W^{t-1}, U^{t-1}, \tilde{X}^t) \\
&=\sum\nolimits_{t=0}^{T-1} I(\bar{X}^t; W_t|W^{t-1}, U^{t-1}, \tilde{X}^t) \\
&=I(\bar{X}^{T-1}\rightarrow W^{T-1}\| U^{T-2}, \tilde{X}^{T-1}) \\
&\stackrel{\text{(d)}}{\geq} I(\bar{X}^{T-1}\rightarrow U^{T-1}\| \tilde{X}^{T-1})
\end{align*}
Inequality (a) is a standard result [Theorem 2.6.4, Cover-Thomas]. Inequality (b) holds since conditioning does not increase entropy, and (c) is because entropy is non-negative. Finally, (d) is due to Lemma~\ref{lemcoding}.



==> casestudy.tex <==
We demonstrate the use of transfer entropy MDPs subject to temporal logic specifications in a scenario based on the upcoming Mars 2020 mission~\cite{landau2015helicopter}. 

Mars rovers operate in mostly unknown environments. Limited a priori knowledge of the terrain and possible obstacles can be provided from low-resolution satellite imagery. This information, however, is often not enough for decision-making as was evidenced by the Curiosity rover which suffered punctures, due to the unexpected presence of jagged, immobile, rocks embedded in the terrain. Proposed methods to reduce damage such as driving the rover backwards requires heavy human intervention and planning. For autonomous decision-making to be viable, information on local terrain characteristics is needed for planning so that manual intervention can be reduced. For the Mars 2020 mission, a helicopter has been proposed to act as a scout \cite{landau2015helicopter} to assist with planning. Figure \ref{fig:mars2020} shows an artists' rendering of the helicopter flying ahead to scout. The helicopter can then transmit information of the terrain back to the rover which is used for planning to satisfy the mission specification. However, transmission costs power, so we are interested in planning to satisfy the mission specification while relying on as little information from the helicopter as possible

\begin{figure}
\centering
\includegraphics[scale=0.36]{mars2020.jpg}
\caption{Artist's rendering of the proposed helicopter to scout for the Mars rover. The helicopter can fly ahead and send information back to the rover about the presence of any obstacles. \cite{landau2015helicopter}.}\label{fig:mars2020}
\end{figure}

We develop tools to address some of the navigation challenges in this mission. The specifics of the experiment is described in Section $\ref{sec:exp}$.

%{\color{blue} JUST SAY BRIEFLY THAT WE DEVELOP TOOLS TO ADDRESS SOME OF NAVIGATION CHALLENGES IN THIS MISSON AND DISCUSS THE REST IN THE EXAWe model a scenario where the rover is tasked with collecting samples from a specific region. The environment is modeled as an MDP as motion can be stochastic, i.e, slippage can occur. The mission is specified in LTL as it allows us to easily and formally state high level tasks for the rover, and the decision-making goal is to \emph{maximize} the probability of satisfying the mission specification. The helicopter can send terrain information (such as locations of any small rocks) to the rover to assist in path planning but transmitting information costs power. We provide a method that allows the planner to maximize the probability of completing the mission while also penalizing information transfer. MPLE SECTION....
%This means the rover must plan to satisfy the mission specification while relying on as little information from the helicopter as possible. The specifics of the experiment is described in section $\ref{sec:exp}$.}

==> comm_rate.tex <==

In this section, we consider a communication-theoretic meaning of the optimization problem \eqref{eqmainproblem}. Consider a feedback control architecture shown in Figure~\ref{fig:NCS}. 


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{comm.pdf}
\caption{Example of a feedback control structure with remote and local sensors}
\label{fig:NCS}
\end{figure}


At every time step $t$, assume that the free component $\tilde{X}_t$ of the state vector is immediately available to the controller, while the expensive component $\bar{X}_t$ is only available at a remote sensor. The remote sensor produces a discrete codeword $W_t\in\mathcal{W}_t$ based on a policy $p_t(w_t|\bar{x}^t, w^{t-1})$, where $\mathcal{W}_t$ is a certain codebook such that $|\mathcal{W}_t|=2^{R_t}$. Codeword is transmitted over a noiseless communication channel and received by the controller without delay, and a control input $U_t$ is generated based on a policy $p_t(u_t|\tilde{x}^t, w^t, u^{t-1})$.
Assuming that transmitting data over the communication channel incurs unit cost $\beta$ per \emph{bit}, consider the following communication design problem
\begin{equation}
\min_{\{\mathcal{W}_t, p_t(w_t|\bar{x}^t, w^{t-1}), p_t(u_t|\tilde{x}^t, w^t, u^{t-1}) \}_{t=0}^{T-1}}  J(X^T, U^{T-1}) +\beta R \label{eqcommproblem}
\end{equation}
where $R=\sum_{t=0}^{T-1}R_t$ is the total amount of data. 
The next result shows that \eqref{eqdi} provides a lower bound to $R$.
\begin{theorem}
\label{theorate}
Suppose that the plant dynamics is given by an MDP $M$. For any choice of the codebook $\mathcal{W}_t$, sensor policy $p_t(w_t|\bar{x}^t, w^{t-1})$ and controller policy $p_t(u_t|\tilde{x}^t, w^t, u^{t-1})$ for $0\leq t\leq T-1$ in Figure~\ref{fig:NCS}, we have
\[
R \geq I(\bar{X}^{T-1}\rightarrow U^{T-1}\| \tilde{X}^{T-1}).
\]
\end{theorem}
\begin{proof}
See Appendix \ref{sec:prf}
\end{proof}
Theorem~\ref{theorate} shows that the optimization problem \eqref{eqmainproblem} provides a fundamental performance limitation of the networked control system shown in Figure~\ref{fig:NCS} in that the optimal value of \eqref{eqcommproblem} is lower bounded by the optimal value of \eqref{eqmainproblem}.




%Consider Figure \ref{fig:NCS}. Assume that transmitting data for $\bar{X}$ over the communication channel incurs unit cost $\beta$ per \emph{bit}, and now consider the following communication design problem
%\begin{equation}
%\min_{\{\mathcal{W}_t, p_t(w_t|\bar{x}^t, w^{t-1}), p_t(u_t|\tilde{x}^t, w^t, u^{t-1}) \}_{t=0}^{T-1}}  J(X^T, U^{T-1}) +\beta R \label{eqcommproblem}
%\end{equation}
%where $R=\sum_{t=0}^{T-1}R_t$ is the total amount of data. 
%The next result shows that \eqref{eqdi} provides a lower bound to $R$.
%\begin{theorem}
%	Suppose that the plant dynamics is given by an MDP $M$. For any choice of the codebook $\mathcal{W}_t$, sensor policy $p_t(w_t|\bar{x}^t, w^{t-1})$ and controller policy $q_t(u_t|\tilde{x}^t, w^t, u^{t-1})$ for $0\leq t\leq T-1$ in Figure \ref{fig:NCS}, we have
%	\[
%	R \geq I(\bar{X}^{T-1}\rightarrow U^{T-1}\| \tilde{X}^{T-1}).
%	\]
%\end{theorem}
%\begin{proof}
%	Appendix.
%\end{proof}

%In this section we present a physical intepretation of the use of transfer entropy in this problem formulation in the case of a networked control problem. We will prove the rate of communication $R(D)$ will be lower bounded by the directed information. We first prove the following lemma.
%\begin{lemma}
%\begin{align}
%I(X_1^T \rightarrow U^T || X_2^T) \leq I(X_1^T \rightarrow W^T || U^{T-1},X_2^T)
%\end{align}
%\end{lemma}
%\begin{proof}
%\begin{align*}
%0 &\leq I(X_1^T \rightarrow U^T || X_2^T) - I(X_1^T \rightarrow W^T || U^{T-1},X_2^T) \\
%& = \sum_{t=1}^T I\left(X_1^t;W_t|W^{t-1},U^{t-1},X_2^t \right) - I\left(X_1^t;U_t|U^{t-1},X_2^t \right)\\
%& = \sum_{t=1}^T I\left(X_1^t;W_t,U_t|W^{t-1},U^{t-1},X_2^t \right) \\&- I\left(X_1^t;U_t|U^{t-1},X_2^t \right)\\
%& = \sum_{t=1}^T I\left(X_1^t;W_t|U^{t},X_2^t \right) - I\left(X_1^t;W^{t-1}|U^{t-1},X_2^t \right)\\
%& = \sum_{t=1}^T I\left(X_1^t;W_t|U^{t},X_2^t \right) - I\left(X_1^{t-1};W^{t-1}|U^{t-1},X_2^{t-1} \right)\\
%& = I\left(X_2^T;W^T | U^T,X_1^T \right) \geq 0 
%\end{align*}
%\end{proof}
%The third line follows from the fact 
%\begin{align*}
% I & \left(X_1^t;W_t,U_t| W^{t-1},U^{t-1}, X_2^t \right) =  \\ & I\left(X_1^t;W_t|W^{t-1},U^{t-1},X_2^t \right) + I\left(X_1^t;U_t|W^{t},U^{t-1},X_2^t \right) = \\ & I\left(X_1^t;W_t|W^{t-1},U^{t-1},X_2^t \right)
%\end{align*}
%The next line follows from using the chain rule. 
%
%We now present one of the main results of the paper. 
%\begin{theorem}
%$R(D) \geq I(X_1^T \rightarrow U^T || X_2^T)$
%\end{theorem}
%
%\begin{proof}
%\begin{align*}
%\sum_{t=1}^T R_t &\geq \sum_{t=1}^T H(W_t)\\
%&\geq \sum_{t=1}^T H(W_t\vert W^{t-1},U^{t-1},X_2^t)\\
%&\geq \sum_{t=1}^T H(W_t\vert W^{t-1},U^{t-1},X_2^t) - H(W_t\vert X_1^t, W^{t-1},U^{t-1},X_2^t)\\
%& =  \sum_{t=1}^T I \left(X_2^T \rightarrow W^T \vert \vert U^{T-1},X_2^{T} \right)\\
%& \geq I \left(X_1^T \rightarrow U^T \vert \vert X_2^T \right)
%\end{align*}
%\end{proof}

==> infotheory.tex <==
Let $M=(\mathcal{X},\mathcal{U},p,\AP,L)$ be a finite labeled MDP.
The \emph{joint distribution} $\mu_{t}(x^{t}, u^{t-1})$ is defined recursively by the state transition probability $p(x_{t+1}|x_t, u_t)$ and a policy $q_t(u_t|x^t, u^{t-1})$ as
\[
\mu_{t+1}(x^{t+1}, u^t)=p_t(x_{t+1}|x_t, u_t)q_t(u_t|x^t, u^{t-1})\mu_t(x^t, u^{t-1}).
\]

Suppose that the state space of $M$ is split such that $\mathcal{X}=\bar{\mathcal{X}}\times \tilde{\mathcal{X}}$. Given random variables $\bar{X},\tilde{X},U$ The \emph{conditional mutual information} is given by 

\begin{align*}
I  (\bar{X}^t;U_t & \vert U^{t-1},\tilde{X}^{t}) \defeq \nonumber \\ &\mathbb{E}_{\mu_T}\bigg\{\log\frac{\mu_{t}(U_t|\bar{X}^{t},U^{t-1},\tilde{X}^t)}{\mu_{t}(U_t\vert U^{t-1}, \tilde{X})^t}\bigg\}.
\end{align*}

We assume that the observation cost over the time horizon $0\leq t\leq T-1$ is proportional to the (causally conditioned) \emph{transfer entropy}.
\begin{equation}
\label{eqdi}
I(\bar{X}^{T-1}\rightarrow U^{T-1}\| \tilde{X}^{T-1})=\sum_{t=0}^{T-1} I(\bar{X}^t; U_t|U^{t-1},\tilde{X}^t).
\end{equation}
We note that the notion of \emph{directed information} is introduced by \cite{massey1990causality} based on \cite{marko1973bidirectional}, and its generalization with causal conditioning by \cite{kramer1998causal}. Intuitively, \eqref{eqdi} can be understood as the information flow from a random process $\{\bar{X}_t\}$ to $\{U_t\}$ given $\{\tilde{X}_t\}$ as side information.

 
%Formally,
%\[
%J(X^T, U^{T-1})=I(\bar{X}^{T-1}\rightarrow U^{T-1}\| \tilde{X}^{T-1}).
%\]
%Suppose that the state space of $M$ is split into the space $\bar{\mathcal{X}}$ of ``expensive to observe'' state variables and the space $\tilde{\mathcal{X}}$ of ``free'' state variables as $\mathcal{X}=\bar{\mathcal{X}}\times \tilde{\mathcal{X}}$.
%At every time step, observing a realization of the ``free'' component $\tilde{X}_t$ of the state random variable $X_t=(\bar{X}_t, \tilde{X}_t)$ is free of charge, whereas observing the ``expensive'' component $\bar{X}_t$ incurs cost. 






==> opt_cond.tex <==
Now, given the optimization problem in equation (\ref{eqn:constopt}), we derive sufficient conditions for optimality for the policy $q_t(u_t|x^t,u^{t-1})$. First, we look at a generalized version of the problem for a single time step. We use that to set up a backwards dynamic programming problem where the generalized version is solved at each step.

\subsection{Generalized static problem}
Let $X_1,X_2,U,Z$ be random variables taking values from sets $\mathcal{X}_1,\mathcal{X}_2,\mathcal{U},\mathcal{Z}$. Let $c : X_1 \times X_2 \times U \times Z \rightarrow \mathbb{R}$ be an arbitrary function. We can treat the optimization problem in (\ref{eqn:nonconstopt}) as a specific case of the following generalized problem

\begin{align}\label{eqn:genopt}
\min_{q(u|x_1,x_2,z)} \mathbb{E}\{c\left(x_1,x_2,u,z \right)\} + I(x_2;a|x_1,z)
\end{align}

\begin{lemma}
It can be shown that a sufficient optimality condition for the above can be written as the \textit{Gibbs distribution}
\begin{align}
q^{*}(u|x_1,x_2,z) = \frac{\nu^{*}(u,x_1|x_2,z)\exp\{-c(x_1,x_2,u,z)\}}{\sum_{u\in \mathcal{U}}\nu^{*}(u,x_1|x_2,z)\exp\{-c(x_1,x_2,u,z)\}}
\end{align}
where 
\begin{align}
\nu^{*}(u,x_1|x_2,z) = \sum_{\mathcal{X}_2}p(x_2|z,x_1)q^*\left(-c(x_1,x_2,u,z)\right)
\end{align}
$p(x_1,x_2,z)-$everywhere.
\end{lemma}

The proof of this is standard and can be found in \cite{petersen2012robust}. We can substitute this into equation (\ref{eqn:genopt}) to express the optimal value as:
\begin{align}\label{eqn:statopt}
-\sum_{\mathcal{X}_2,\mathcal{Z}}\log\left\lbrace\sum_{\mathcal{U}} \nu^{*}(u,x_1|x_2,z)\exp\{ -c(x_1,x_2,u,z)\} \right\rbrace
\end{align}
We define partition function
\begin{align}
\phi^{*}(x_1,x_2,z) =  \sum_{\mathcal{U}} \nu^{*}(u,x_1|x_2,z)\exp\{ -c(x_1,x_2,u,z)\} 
\end{align}
and rewrite equation (\ref{eqn:statopt}) as 
\begin{align}
\mathbb{E}^{p(x_2,z)}\left\lbrace\log\{\phi^{*}(x_1,x_2,z) \}\right\rbrace
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Dynamic programming}
Recall that $\mu_t(x_1^t, x_2^t,u^{t-1})$ is the joint distribution of states and actions. We define the \emph{cost-to-go} function as

\begin{align}
V_t(\mu_t(x_1^t,& x_2^t,u^{t-1}))  \defeq \nonumber \\
& \min_{q_{k=t}^T} \sum_{t=1}^{T}\{ \mathbb{E}\{c_t\left(x_{1_t},x_{2_t},u_t \right)\} + I(x_1^t;u^t|u^{t-1},x_2^t) \}
\end{align}
This is the \textit{value} of the current \emph{configuration} $\mu_t(x_1^t, x_2^t,u^{t-1})$.

This cost-to-go function must satisfy the Bellman equation given by:
\begin{align}
V_t(\mu_t(x_1^t,& x_2^t,u^{t-1})) \defeq \nonumber \\ 
& \min_{q_t} \left\lbrace \mathbb{E}^{q_t,\mu_t}\left\lbrace c_t(X_{1}^t,X_{2}^t,U_t) + I(X_1^t,U_t \vert X_{2}^t,U^{t-1} \right\rbrace) \right\rbrace
\end{align}

\begin{align}
V_t(\mu_t(x_1^t,& x_2^t,u^{t-1})) \defeq \nonumber \\ 
& \min_{q_t} \{ \mathbb{E}\{\rho_t\left(x_{1_t},x_{2_t},u_t \right)\} + I(x_1^t;u^t|u^{t-1},x_2^t) \}
\end{align}
where 
\begin{align}
\rho_t\left(x_{1_t},x_{2_t},u^t\right) & \defeq  c_t\left(x_{1_t},x_{2_t},u_t\right) - \nonumber \\ & \sum_{X_{t+1}}p_{t+1}(x_{t+1}|x_t,u_t)\log \phi_{t+1}(x_{t+1},u^t)
\end{align}

In the standard finite-state MDP setting, the Bellman equation for the cost-to-go function is solved using backwards dynamic programming by evaluating the value function in the entire state space of the MDP. However, this is not feasible in our setting as our state space consists of the space of probability distributions $\mu_t(x_1^t, x_2^t,u^{t-1})$ which is not finite.  

From the previous section, we know the sufficient optimality condition for a candidate solution $q^{*}$ for an optimization problem of the given form is:
\begin{align}
q_t^{*}(a_t|s_1^t,s_2^t,a^{t-1}) = \frac{\nu_t^{*}(a_t|s_2^t,a^{t-1})\exp\{-\rho_t\left(s_{1_t},s_{2_t},a^t\right)  \}}{\sum_{u \in \mathcal{U}} \nu_t^{*}(a_t|s_2^t,a^{t-1})\exp\{-\rho_t\left(s_{1_t},s_{2_t},a^t\right)  \}}
\end{align}
where 


\begin{align}
\nu_t^{*}(a_t|s_2^t,a^{t-1}) = \sum_{S_1^t}q_t^{*}(a_t|s_1^t,s_2^t,a^{t-1})\mu_t(s_1^t|s_2^t,a^{t-1})
\end{align}


==> problem_Takashi.tex <==
Consider the control system architecture shown in Figure \ref{fig:NCS} modeled by a finite state discrete-time MDP. The state space $\mathcal{X}$ is composed of the product of two sets  $\mathcal{X} = \mathcal{X}_e \times \mathcal{X}_f$. Hence, each state in the state space $x \in \mathcal{X}$ is partitioned into two state variables $x = (x_e,x_f)$. Recall that a policy is a conditional policy distribution given by $q(u_t|x^t,u^{t-1})$. We can write this now as $q(u_t|x_e^t,x_f^t,u^{t-1})$. We allow the policy synthesizer full access to the value of $x_f$, but we restrict access to the value of $x_e$. As a motivating scenario, imagine the MDP models a Mars rover. The value of $x_e$ is measured by an orbiter while $x_f$ is sensed using on-board sensors. Since the orbiter will only be able to communicate with the rover during part of its orbit, we will want to penalize the reliance on this information in the policy synthesis process. To do this we introduce some information-theoretic terms. 



Let $X_e \in \mathcal{X}_e,X_f \in \mathcal{X}_f,U\in \mathcal{U}$ be random variables of which $x_e,x_f,u$ are realizations. The \emph{conditional mutual information} is 

\begin{align*}
I  (X_{e_{t-m}}^t;U_t & \vert U^{t-1}_{t-n},X_{f_{t-m}}^{t}) \defeq \nonumber \\ &\sum_{\mathcal{X}^{t}_f}\sum_{\mathcal{U}^{t-1}}\log\frac{\mu_{t+1}(u_t|x_{t-m}^{t},u_{t-n}^{t-1})}{\mu_{t+1}(u_t\vert u_{t-n}^{t-1})}
\end{align*}\todo{Fix definition}



The transfer entropy of degree $(m,n)$ is defined as \cite{schreiber2000}

\begin{align}\label{eqn:TEcond}
I_{m,n}(X_e^T  \rightarrow & U^{T-1}||X_f^T) \defeq \nonumber \\ & \sum_{t=0}^{T-1} I\left(X_{e_{t-m}}^t;U_t|U^{t-1}_{t-n},X_{f_{t-m}}^{t} \right) .
\end{align}





% An \emph{encoder} and \emph{decoder} are defined as stochastic kernels $e_t(w_t|x^t,w^{t-1})$ and $d_t(u_t|w^t,u^{t-1})$ respectively. $w_t$ is a \emph{codeword} chosen from \emph{codebook} $\mathcal{W}_t$ at time $t$. $|\mathcal{W}_t| = 2^{R_t}$. $R = \sum_{t=1}^T$ is the rate of communication. 

% For example in Figure \ref{fig:NCS}, at each time step the sensor sends data to the encoder which chooses a codeword $w_t$ and passes the message to the decoder. 


% \paragraph{Optimal policy}
% Given an MDP $M=(\mathcal{X},\mathcal{U},p)$ with cost function $c_t: \mathcal{X} \times \mathcal{U} \rightarrow \mathbb{R}$, and finite time horizon $T$, the optimal policy $q$ is one that minimizes the following

% \begin{equation}\label{eqn:optpol}
% J(X^T,U^{T-1}) \defeq \sum_{t=0}^{T-1}{\mathbb{E}\{c_t(X_t,U_t)\}} + \mathbb{E}\{c_{T}(X_{T})\}
% \end{equation}

% Informally, the policy minimizes the expected value of the cost over the time horizon. In this setting the optimal policy will be deterministic and Markovian. 

% \paragraph{Expensive-to-measure state variable} We divide the state space $\mathcal{X}$ into expensive and free to measure state variables, \ie $\mathcal{X} = \mathcal{X}_e \times \mathcal{X}_f$. A state $x \in \mathcal{X}$ can be expressed as $x = (x_e,x_f)$ where $x_e \in \mathcal{X}_e$ is expensive-to-measure and $x_f \in \mathcal{X}_f$ is free. 

% Now, consider the following information-constrained optimal control problem:
% \begin{equation}
% \min_{\{q_t\}_{t=1}^T} J(X^{T},U^{T-1}) + \beta \sum_{t=0}^T R_t
% \end{equation}
% where $\beta \in \mathbb{R}$, $R = \sum_{t=0}^T R_t$ is the rate of communication, and $J(X^T,U^{T-1}) \defeq \sum_{t=0}^{T-1}{\mathbb{E}\{c(X_t,U_t)\}} + \mathbb{E}\{c_{T}(X_{T})\}$ for some state-action dependent cost $c(X_t,U_t) \in \mathbb{R}$. 

\begin{figure}
\centering
\begin{tikzpicture}[auto, node distance=2cm,>=latex']
    % We start by placing the blocks
    \node [input, name=input] {};
    \node [sum, right of=input] (sum) {};
    \node [block, right of=sum,text width=2.1cm] (controller) {\textbf{Controller}\\$q_t(u_t|x^t,u^{t-1})$};
    \node [block, right of=controller,node distance = 3cm,text width=2cm] (dynamics) {\textbf{Dynamics}\\$p(x_{t+1}|x_t,u_t)$};
    % We draw an edge between the controller and system block to 
    % calculate the coordinate u. We need it to place the measurement block. 
    \node [output, right of=dynamics] (output) {};
    \node [sblock, below of=dynamics,text width = 1cm] (xc) {\textbf{Sensor}\\$x_c$};
    \node [sum, left of=xc] (encoder) {e};
	\node [sblock, below of=xc,node distance = 1.5cm, text width = 1cm] (xf) {\textbf{Sensor}\\$x_f$};
	\node [sum, below of=controller,node distance = 1.3cm] (decoder) {d};
    % Once the nodes are placed, connecting them is easy. 
    \draw [draw,->] (input) -- node {$r$} (sum);
    \draw [->] (sum) -- node {$e$} (controller);
    \draw [->] (controller) -- node {$u$} (dynamics);
    \draw [->] (dynamics) -- node [name=y] {$y$}(output);
    \draw [->] (y) |- (xc);
    \draw [->] (xc) -- (encoder);
    \draw [->] (y) |- (xf);
    \draw [->] (encoder) -- (decoder);
     \draw [->] (decoder) -- (sum);
    \draw [->] (xf) -| node[pos=0.99] {$-$} 
            node [near end] {}(sum);
\end{tikzpicture}\caption{Control system architecture where $x_e$ is sensed remotely and has to be transmitted to the controller through an encoder-decoder system.}\label{fig:NCS}

\end{figure}

